UTBoost: Gradient Boosted Decision Trees for Uplift Modeling

Uplift modeling comprises a collection of machine learning techniques designed for managers to predict the incremental impact of specific actions on customer outcomes. However, accurately estimating this incremental impact poses significant challenges due to the necessity of determining the difference between two mutually exclusive outcomes for each individual. In our study, we introduce two novel modifications to the established Gradient Boosting Decision Trees (GBDT) technique. These modifications sequentially learn the causal effect, addressing the counterfactual dilemma. Each modification innovates upon the existing technique in terms of the ensemble learning method and the learning objective, respectively. Experiments with large-scale datasets validate the effectiveness of our methods, consistently achieving substantial improvements over baseline models.

==> content/abstract.tex <==
Uplift modeling comprises a set of machine learning techniques that enable managers to predict the incremental impact of an action on specific customer outcomes. 
These models empower decision-makers to identify customer segments most likely to respond positively to particular interventions, thus optimizing the allocation of resources and maximizing overall gains. 
However, accurately estimating this incremental impact poses significant challenges due to the necessity of determining the difference between two mutually exclusive outcomes for each individual. 
In our study, we introduce two innovative modifications to the established Gradient Boosting Decision Trees (GBDT) technique. 
These modifications sequentially learn the causal effect, addressing the counterfactual dilemma. 
Each approach innovates upon the existing technique in terms of the ensemble learning method and the learning objective, respectively. 
Experiments with large-scale datasets validate the effectiveness of our methods, consistently achieving substantial improvements over baseline models.

